Consistent Query Answering for Expressive Constraints under Tuple-Deletion Semantics

We study consistent query answering in relational databases. We consider an expressive class of schema constraints that generalizes both tuple-generating dependencies and equality-generating dependencies. We establish the complexity of consistent query answering and repair checking under tuple-deletion semantics for different fragments of the above constraint language. In particular, we identify new subclasses of constraints in which the above problems are tractable or even first-order rewritable.

==> 3-old-preliminaries.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Preliminaries}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ineq}{\gamma}
\newcommand{\bodyp}{\body_p}
\newcommand{\headp}{\head_p}
\newcommand{\notequal}{\textit{NotEq}}
\newcommand{\checknotffk}{\textit{CheckNot\ffk}}
\newcommand{\bcq}{\textit{BCQ}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Databases, Dependencies and Queries}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A \emph{DB schema} $\S$ is a predicate signature, i.e., a set of predicate symbols with an associated arity. We assume that a predicate signature always contains the special predicate $\bot$ of arity 0.
%
A \emph{DB instance} $\D$ (or simply \emph{database}) for $\S$ is set of facts (i.e., ground atoms) over the predicates of $\S$.

A \emph{term} is either a variable symbol or a constant symbol.
%
A \emph{predicate atom} (or simply \emph{atom}) is an expression of the form $p(t)$, where $p$ is a predicate of arity $n$ and $t$ is a $n$-tuple of terms.
%
An \emph{inequality} (or just \emph{inequality}) is an expression of the form $t\neq t'$, where $t$ and $t'$ are terms.

\begin{definition}[Dependency]\label{def:dependency-new}
    Given a DB schema $\S$, a \emph{dependency} for $\S$ is a first-order sentence over the predicates of $\S$ of the form:
    $$\forall x\, (\alpha_1\wedge\ldots\wedge\alpha_k\wedge\ineq_1\wedge\ldots\wedge\ineq_h \rightarrow\exists y\, (\beta_1\wedge\ldots\wedge\beta_m\wedge\ineq_1'\wedge\ldots\wedge\ineq_\ell'))$$
    where $k\geq 1$, $h\geq 0$, $m\geq 1$, $\ell\geq 0$, $x$ and $y$ are vectors of variables, every $\alpha_i$ is a predicate atom such that every variable occurring in $\alpha_i$ also occurs in $x$,
    every variable of $x$ occurs in at least one predicate atom $\alpha_i$,
    every $\beta_i$ is a predicate atom such that every variable occurring in $\beta$ also occurs either in $x$ or in $y$,
    every $\ineq_i$ is an inequality of the form $t\neq t'$ where $t,t'$ are either constants or variables from $x$,
    and every $\ineq_i'$ is an inequality of the form $t\neq t'$ where $t,t'$ are either constants or variables from $x,y$.
\end{definition}

Given a dependency $\tau$ of the above form, we denote by $\body(\tau)$ the formula $\alpha_1\wedge\ldots\wedge\alpha_k\wedge\ineq_1\wedge\ldots\wedge\ineq_h$, and denote by $\head(\tau)$ the formula $\beta_1\wedge\ldots\wedge\beta_m\wedge\ineq_1'\wedge\ldots\wedge\ineq_\ell'$.
%%
We also denote by $\bodyp(\tau)$ the set of predicate atoms $\{\alpha_1,\ldots,\alpha_k\}$, and denote by $\headp(\tau)$ the set of predicate atoms $\{\beta_1,\ldots,\beta_m\}$.
%% We also denote by $\bodyp(\tau)$ the formula $\alpha_1\wedge\ldots\wedge\alpha_k$, and denote by $\headp(\tau)$ the formula $\beta_1\wedge\ldots\wedge\beta_m$.
%%
With a slight abuse of notation, we write $\alpha\in\body(\tau)$ (respectively, $\alpha\in\head(\tau)$) to denote that the atom $\alpha$ occurs in the conjunction $\body(\tau)$ (respectively, $\head(\tau)$).
%%
Moreover, we call \emph{frontier variables of $\tau$} the variables of $\tau$ occurring both in $\body(\tau)$ and in $\head(\tau)$. 

\warn{(*** FORSE DOBBIAMO ESCLUDERE DALLE FRONTIER LE VAR CHE NELLA TESTA COMPAIONO SOLO NELLE DISUGUAGLIANZE!!??***)}

Let $\conj=\alpha_1\wedge\ldots\wedge\alpha_k\wedge\ineq_1\wedge\ldots\wedge\ineq_h$ be a conjunction of predicate atoms and inequalities. An \emph{instantiation of $\conj$ in $\D$} is a substitution $\sigma$ of the variables occurring in $\conj$ with constants such that 
%% every ground atom occurring in the conjunction $\sigma(\conj)$ belongs to $\D$.
$(i)$ $\sigma(\alpha_i)\in\D$ for every $i$ such that $1\leq i\leq k$;
$(ii)$ none of the inequalities $\sigma(\ineq_1)\ldots\wedge\sigma(\ineq_h)$ has the form $t\neq t$ (where $t$ is either a constant or a variable).
%%
Moreover, given an instantiation $\sigma$ of $\conj$ in $\D$, we call \emph{image of $\conj$ in $\D$} the subset $\{\sigma(\alpha_1),\ldots,\sigma(\alpha_k)\}$ of $\D$.

A dependency $\tau$ is \emph{satisfied} by a database $\D$ if, for every instantiation $\sigma$ of $\body(\tau)$ in $\D$, there exists at least one instantiation of $\head(\sigma(\tau))$ in $\D$.

\begin{definition}[Consistency and Weak consistency]
Given a set of dependencies $\constr$, we say that a database $\D$ is \emph{consistent with $\constr$} if all the dependencies of $\constr$ are satisfied in $\D$. Moreover, we say that a subset $\D'$ of $\D$ is \emph{weakly consistent with $\SD$} if there exists a subset $\D''$ of $\D$ such that $\D'\subseteq\D''$ and $\D''$ is consistent with $\constr$.
\end{definition}

% \warn{***SONO VERAMENTE ANCORA NECESSARIE LE SEGUENTI DEFINIZIONI DI VIOLATION?? SEMBRA PROPRIO DI NO***}

% \begin{definition}[Weak violation]
% Given a set of facts $\D'$, a \emph{weak violation of $\Sigma$ in $\D'$} is a subset $\D''$ of $\D'$ such that $\D''$ is an image of the body of a dependency $\tau$ in $\Sigma$ such that, for each instantiation $\sigma$ of $\body(\tau)$ in $\D''$,
% $(i)$ $\sigma(\head(\tau))$ has no image in $\D''$ and
% $(ii)$ $\sigma(\head(\tau))$ has an image in $\D'$.
% \end{definition}

% \begin{definition}[Violation]
% Given a database $\D$ and a set of dependencies $\constr$, a \emph{violation of $\SD$} is a subset $\D'$ of $\D$ such that there exists an instantiation $\sigma$ of $\body(\tau)$ in $\D'$ such that $\sigma(\head(\tau))$ has no image in $\D$.
% \end{definition}

% \begin{proposition}
% \label{pro:consistent-violations}
% A set of facts $\D'$ is consistent with $\Sigma$ iff $\D'$ does not contain any violation of $\tup{\Sigma,\D'}$ and does not contain any weak violation of $\Sigma$ in $\D'$.
% \end{proposition}

% \begin{proposition}
% \label{pro:weakly-consistent-violations}
% A set of facts $\D' \subseteq \D$ is weakly consistent with $\SD$ iff $\D'$ does not contain any violation of $\SD$.
% \end{proposition}

\begin{definition}[BCQ and BUCQ]\label{def:bcq}
    A \emph{Boolean conjunctive query with inequalities (BCQ)} is a first-order sentence of the form:
    \begin{equation}
    \label{eqn:bcq}    
    \exists x\, (\alpha_1\wedge\ldots\wedge\alpha_k\wedge\gamma_1\wedge\ldots\wedge\gamma_h)
    \end{equation}
    where every $\alpha_i$ is a predicate atom such that every variable occurring in $\alpha_i$ also occurs in $x$, and every $\gamma_i$ is an inequality on constants or variables from $x$.
    %%
    A \emph{Boolean union of conjunctive queries with inequalities (BUCQ)} is a first-order sentence of the form $\bigvee_{i=1}^m q_i$, where each $q_i$ is a BCQ.
\end{definition}

We denote by $\bcq(Q)$ the set of BCQs occurring in a BUCQ $Q$ (i.e.\ if $\bigvee_{i=1}^m q_i$ then $\bcq(Q)=\{q_1,\ldots,q_m\}$).
%%
Given a BCQ $q$ of the above form (\ref{eqn:bcq}) and a database $\D$, we call \emph{image of $q$ in $\D$} every image of $\alpha_1\wedge\ldots\wedge\alpha_k\wedge\gamma_1\wedge\ldots\wedge\gamma_h$ in $\D$, and given a BUCQ $Q$, we call \emph{image of $Q$ in $\D$} every image of every BCQ $q_i\in\bcq(Q)$ in $\D$.
%%
Moreover, we say that $Q$ \emph{has an image in $\D$} if there exists $q\in\bcq(Q)$ such that $q$ has an image in $\D$.
%% If $q$ has an image in $\D$, we write $\D\models q$.

For some results presented in this paper, it is important to keep in mind that the images of a BCQ with $k$ predicate atoms in a database $\D$ are at most $n^k$ (where $n=|\D|$) and can be computed in polynomial time \wrt data complexity.
%%
% In this case, we write $\sigma(q)=\D'$. Moreover, we say that $q$ has an image in a database $\D$ if there exists $\D'\subseteq\D$ such that $\D'$ is an image of $q$.

Dependencies and BUCQs are subclasses of the class of domain-independent relational calculus sentences \cite{AHV95}. 
%% 
Given a domain-independent sentence $\phi$ of the relational calculus, we write $\D\models\phi$ if the evaluation of $\phi$ over $\D$ is true.
%%
It is immediate to verify that, for a BUCQ $Q$, $\D\models q$ iff $q$ has an image in $\D$ and that, for a set of dependencies $\Sigma$, $\D$ is consistent with $\Sigma$ iff $\D\models\bigwedge_{\tau\in\Sigma}\tau$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Subclasses of dependencies}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We say that a dependency is \emph{linear} in the case when $k=1$.

When $y$ is empty, we say that the dependency is \emph{full}.

% Given a DB schema $\S$, a database $\D$ for $\S$, and an $n$\nobreakdash-ary predicate $p$ of $\S$, we say that a set of arguments %$\Lambda$
% $a_1,\ldots,a_m$ (with $m \le n$) is a \emph{factual key} for $p$ in $\D$ if there do not exist two distinct facts $p(c_1,\ldots,c_n)$ and $p(c'_1,\ldots,c'_n)$ in $\D$ %such that $c_i=c'_i$ for each argument of $\Lambda$.\\
% whose projections \wrt $a_1,\ldots,a_m$ coincide.

Given a database $\D$ for $\S$, and a dependency $\tau$ for $\S$, we say that $\tau$ is \emph{forward-deterministic (\ffk) for $\D$} if, for every instantiation $\sigma$ of $\body(\tau)$ in $\D$, there exists at most one instantiation of $\sigma(\head(\tau))$ in $\D$.
%%
Moreover, we say that a set of dependencies $\Sigma$ is \emph{\ffk for $\D$} if every dependency of $\Sigma$ is \ffk for $\D$.

It is straightforward to see that full dependencies are forward-deterministic independently of the database $\D$. For non-full set of dependencies $\Sigma$, deciding whether $\Sigma$ is \ffk for a database $\D$ is not a hard task.

\begin{proposition}
\label{pro:ffk-check}
Deciding whether $\Sigma$ is \ffk for $\D$ is in $\aczero$ \wrt data complexity.
\end{proposition}
\begin{proof}
First, observe that $\Sigma$ is not \ffk for $\D$ iff there exists $\tau\in\Sigma$ and an instantiation $\sigma$ of $\body(\tau)$ in $\D$ such that there exists at least two instantiations of $\sigma(\head(\tau))$ in $\D$.
%%
Now let $\checknotffk(\Sigma)$ be the following first-order sentence:
\[
\begin{array}{l}
\displaystyle
\bigvee_{\tau\in\Sigma} \exists x\, \big(\body(\tau)\wedge \exists y\,(\head(\tau)\wedge\exists y'\,(\head'(\tau)\wedge\notequal(y,y')))\big)
\end{array}
\]
where:
%%
$x$ are all the universally quantified variables of $\tau$;
%%
$y$ are all the existentially quantified variables of $\tau$ (i.e.\ the variables appearing only in the head of $\tau$);
%%
$y'$ are a copy of all the existentially quantified variables of $\tau$, and $\head'(\tau)$ is obtained from $\head(\tau)$ by replacing every variable $y_i$ from $y$ with the corresponding copy variable  $y_i'$;
%%
$\notequal(y,y')$ is the formula
\[
(y_1\neq y_1' \vee y_2\neq y_2' \vee\ldots\vee y_m\neq y_m')
\]
Now, it is immediate to verify that $\D\models\checknotffk$ iff $\Sigma$ is not \ffk for $\D$. Consequently, the thesis follows. 
\end{proof}

Let $\S$ be a DB schema and $\constr$ be a set of dependencies for $\S$.
%%
We call \emph{dependency graph} of $\Sigma$ the directed graph $G(\Sigma)$ whose vertices are the dependencies of $\Sigma$ and such that there is one edge from the vertex $\tau_1$ to $\tau_2$ iff the head of $\tau_1$ contains an atom whose predicate appears in a predicate atom of the body of $\tau_2$. We say that $\constr$ is \emph{acyclic} if there is no cyclic path in $G(\Sigma)$.
%%
Given an acyclic set of dependencies $\Sigma$, we call \emph{topological order of $\Sigma$} any topological order of $G(\Sigma)$, i.e.\ a sequence $\tup{\tau_1,\ldots,\tau_h}$ of the dependencies of $\Sigma$ such that, if $i\geq j$, then the vertex $\tau_i$ is not reachable from the vertex $\tau_j$ in $G(\Sigma)$.

%% We call \emph{dependency graph} of $\Sigma$ the directed graph $G$ whose vertices are the predicates of $\S$ and such that there is one edge from the vertex $p_b$ to $p_h$ iff $\constr$ contains a dependency whose body (resp., head) contains an atom whose predicate is $p_b$ (resp., $p_h$). Moreover, we say that $\constr$ is \emph{acyclic}~\cite{AHV95} if there is no cyclic path in $G$.


% \begin{definition}[EGDs]\label{def:egd}
%     Given a DB schema $\S$, an \emph{equality-generating dependency (EGD)} for $\S$ is a first-order formula over the predicates of $\S$ of the form:
%     $$\forall x. \alpha_1\wedge\ldots\wedge\alpha_k\wedge\gamma_1\wedge\ldots\wedge\gamma_h \rightarrow\bot$$
%     where $x$ is a vector of variables, every $\alpha_i$ (resp., $\gamma_i$) is an atom (resp., an inequality) such that every variable occurring in it also occurs in $x$.
% \end{definition}
%In the case $h=0$, an EGD is also called a \emph{denial}.
%Also comparison predicates could be added without changing the complexity results.

From now on, we will omit that databases and dependencies are given for a DB schema $\S$.

%% ***INTRODURRE I TRE CASI MISTI?? acyclic \ffk + acyclic linear, acyclic \ffk + \ffk linear, acyclic \ffk + linear ??

\iflong
In this article we refer to the following computational complexity classes:
\begin{itemize}
    \item $\aczero$, the set of problems solvable by a logspace-uniform family of circuits $\{C_n\}$, where $C_n$ has size $O(n^c)$ for some constant $c>0$ and depth $O(1)$, and gates are allowed to have unbounded fan-in;
    \item NL (or NLOGSPACE), the set of problems solvable in logarithmic space by a non-deterministic Turing machine;
    \item PTIME, the set of problems solvable in polynomial time by a deterministic Turing machine;
    \item NP, the set of problems solvable in polynomial time by a non-deterministic Turing machine;
    \item coNP, the set of problems whose complement is solvable in polynomial time by a non-deterministic Turing machine;
    \item $\pidue$, the set of problems whose complement is solvable in polynomial time by a non-deterministic Turing machine augmented by an oracle for some NP-complete problem.
\end{itemize}
These classes are such that $\aczero\subset\nlogspace\subseteq\text{PTIME}\subseteq\text{NP}\cup\text{coNP}\subseteq\pidue$. 
\else
We assume the reader to be familiar with the computational complexity classes mentioned in this work. For a detailed description, we refer them to the article's extended version.
\fi
Given a complexity class $C$ and a decision problem $p$, we say that $p$ is \emph{$C$-hard} if there exists a logspace reduction from every other problem in $C$ to $p$. Moreover, if $p$ does also belong to $C$, we say that $p$ is \emph{$C$-complete}.

